Comfort and Sickness while Virtually Aboard an Autonomous Telepresence Robot

In this paper, we analyze how different path aspects affect a user's experience, mainly VR sickness and overall comfort, while immersed in an autonomously moving telepresence robot through a virtual reality headset. In particular, we focus on how the robot turns and the distance it keeps from objects, with the goal of planning suitable trajectories for an autonomously moving immersive telepresence robot in mind; rotational acceleration is known for causing the majority of VR sickness, and distance to objects modulates the optical flow. We ran a within-subjects user study (n = 36, women = 18) in which the participants watched three panoramic videos recorded in a virtual museum while aboard an autonomously moving telepresence robot taking three different paths varying in aspects such as turns, speeds, or distances to walls and objects. We found a moderate correlation between the users' sickness as measured by the SSQ and comfort on a 6-point Likert scale across all paths. However, we detected no association between sickness and the choice of the most comfortable path, showing that sickness is not the only factor affecting the comfort of the user. The subjective experience of turn speed did not correlate with either the SSQ scores or comfort, even though people often mentioned turning speed as a source of discomfort in the open-ended questions. Through exploring the open-ended answers more carefully, a possible reason is that the length and lack of predictability also play a large role in making people observe turns as uncomfortable. A larger subjective distance from walls and objects increased comfort and decreased sickness both in quantitative and qualitative data. Finally, the SSQ subscales and total weighted scores showed differences by age group and by gender.

==> defs.tex <==


%% Use this to make index entries appear in the margin
%\usepackage{showidx}

%\usepackage[dvips,ps2pdf]{hyperref} 
%\usepackage{hyperref} 




%% Turn on/off math bold
\def\mbon{\mathversion{bold}}
\def\mboff{\mathversion{normal}}

%% Continuous-time definitions
\def\tf{{\phi}} %% State transition function

\def\queue{{Q}}

%% Nature actions
\def\nata{{\theta}}
\def\natas{{\Theta}} % All nature actions

\def\Xappr{{\hat{X}}} % Approximate state space
\def\Xfappr{{\tilde{X}}} % Approximate state space

%% Borrowed from Devin Balkcom and Matt Mason (ijrr 02 paper):
\newcommand{\FF}[0]{\ensuremath{\Uparrow}}
\newcommand{\BB}[0]{\ensuremath{\Downarrow}}
\newcommand{\LL}[0]{\ensuremath{\curvearrowleft}}
\newcommand{\RR}[0]{\ensuremath{\curvearrowright}}

\def\graph{{\cal G}}

\def\stages{{\cal K}}

\def\histy{{\tilde{y}}} %% History
\def\histu{{\tilde{u}}} %% History
\def\histv{{\tilde{v}}} %% History
\def\histx{{\tilde{x}}} %% History
\def\histz{{\tilde{z}}} %% History
\def\histp{{\tilde{p}}} %% History
\def\histe{{\tilde{e}}} %% History
\def\histtheta{{\tilde{\theta}}} %% History
\def\histyt{{\tilde{y}_t}} %% History
\def\histut{{\tilde{u}_t}} %% History
\def\histxt{{\tilde{x}_t}} %% History
\def\histthetat{{\tilde{\theta}_t}} %% History
\def\histpsit{{\tilde{\psi}_t}} %% History
\def\hspacey{{\tilde{Y}}} %% History
\def\hspaceu{{\tilde{U}}} %% History
\def\hspacex{{\tilde{X}}} %% History
\def\histpt{{\tilde{p}_t}} %% History
\def\histist{{\tilde \ist}}
\def\histq{{\tilde q}}
\def\histplan{{\tilde\plan}}

%% Information space notation
\def\ic{{\eta_0}} %% Initial condition
\def\ics{{{\cal I}_0}} %% Initial condition space
\def\ici{{\eta^i_0}} %% Initial condition
\def\icsi{{{\cal I}^i_0}} %% Initial condition space
\def\ist{{\eta}} %% Information state
\def\istder{{\eta_{der}}} %% Information state
\def\ifs{{\cal I}} %% An information space
\def\ifsder{{\cal I}_{der}} %% History information space
\def\ifsderp{{\cal I}'_{der}} %% History information space
\def\ifsest{{\cal I}_{est}} %% History information space
\def\ifshist{{\cal I}_{hist}} %% History information space
\def\ifsndet{{\cal I}_{ndet}} %% Nondeterministic information space
\def\ifsprob{{\cal I}_{prob}} %% Probabilistic information space
\def\ifsgauss{{\cal I}_{gauss}} %% Probabilistic information space
\def\ifsapp{{\cal I}_{app}} %% Probabilistic information space
\def\ifsmom{{\cal I}_{mom}} %% Probabilistic information space
\def\ifsk{{{\cal I}_k}} %% Native information space
\def\ifst{{{\cal I}_t}} %% Native information space
\def\imap{{\kappa}}
\def\imapndet{{\imap_{ndet}}}
\def\imapprob{{\imap_{prob}}}
\def\imapstage{{\imap_{stage}}}
\def\imapapp{{\imap_{app}}}
\def\imapmom{{\imap_{mom}}}
\def\imapgauss{{\imap_{mom}}}
\def\imapsf{{\imap_{sf}}}
\def\cifs{\ifs_c} %% Collapsed information space
\def\cist{\eta^c} %% Information space
\def\mifs{{\kappa}}
\def\imifs{{\Gamma^{-1}}}
\def\allp{{\Pi}} %% All plans
\def\allpc{{\Pi_\kappa}} %% All plans
\def\ite{{f_\ifs}} %% Information transition equation
\def\iteder{{f_\ifs}_{der}} %% Information transition equation
\def\hplan{{\cal H}} %% Information space
\def\difs{{\cal I}_\imap} %% Information space

\def\infX{{\vec{X}}}
\def\infx{{\vec{x}}}
\def\infU{{\vec{U}}}
\def\infu{{\vec{u}}}
\def\infTheta{{\vec{\Theta}}}
\def\inftheta{{\vec{\theta}}}
\def\inff{{\vec{f}}}
\def\infL{{\vec{L}}}
\def\infl{{\vec{l}}}


\def\Land{{\cal L}}

\def\ehat{\hat{e}}
\def\Ehat{\hat{E}}

\def\utility{{\cal U}}

% D^* definitions

\def\Gbest{{G_{best}}}
\def\Gcur{{G_{cur}}}
\def\Gvia{{G_{via}}}


%% This can be redef'ed later to be whatever we want for the robot
\def\A{{\cal A}}

%% Homeomorphism
\def\homeo{{ \;\cong\; }}

%%% The configuration space?
%\def\Q{{\cal Q}}

\def\choose#1#2{{(^{#1}_{#2})}}

\def\sgn{{\rm sgn}}
\def\sgnv{{\rm sgn}}

\def\pow{{\rm pow}}

\def\pdf{{p}}

%% closed chains
\def\Cclo{{{\cal C}_{clo}}}
\def\Cfea{{{\cal C}_{fea}}}


%% manip
\def\Csta{{{\cal C}_{sta}}}
\def\Cgr{{{\cal C}_{gr}}}
\def\Ctra{{{\cal C}_{tra}}}
\def\Cadm{{{\cal C}_{adm}}}
\def\Caobs{{{\cal C}^a_{obs}}}
\def\Cpobs{{{\cal C}^p_{obs}}}
\def\Capobs{{{\cal C}^{ap}_{obs}}}
\def\Xsta{{X_{sta}}}
\def\Xgr{{X_{gr}}}
\def\Xtra{{X_{tra}}}
\def\Ccon{{{\cal C}_{con}}}
\def\motcom{{\mu}}
\def\allmotcom{{\cal M}}


%%time var
\def\tva{{\tau}}
\def\tvb{{\sigma}}
\def\tvc{{\phi}}
\def\tvd{{g}}

%% multi
\def\multa{{\tau}}
\def\multb{{h}}
\def\cubesim{{\square}}

%% Conformation stuff
\def\confv{{q}}

%% General transformation
\def\gt{{h}}
\def\gti{{h^{-1}}}

%% Translation parameters
\def\xt{x_t}
\def\yt{y_t}
\def\zt{z_t}

%% Logical predicates
\def\lpred{\phi}
\def\qfpred{\phi}
\def\plpred{\alpha}
\def\quant{{\cal Q}}
\def\tarsk{\Phi}
\def\qftask{\phi}
\def\polys{{\cal F}} % Set of polynomials
\def\proot{{\beta}} % Polynomial root

%% Canny's method
\def\polyf{{\psi}}
\def\cmap{{h}}

%% C-space definitions
\def\C{{\cal C}}
\def\Cobs{{\cal C}_{obs}}
\def\Cfree{{\cal C}_{free}}
\def\CP{{P}}
\def\qinit{{q_{I}}}
\def\qgoal{{q_{G}}}
\def\qcur{{q_{cur}}}
\def\qnew{{q_{new}}}
\def\qiinit{{q^i_{I}}}
\def\qigoal{{q^i_{G}}}
\def\qoneinit{{q^1_{I}}}
\def\qonegoal{{q^1_{G}}}
\def\qminit{{q^m_{I}}}
\def\qmgoal{{q^m_{G}}}

\def\Xobs{{X_{obs}}}
\def\Xfree{{X_{free}}}
\def\Xcon{{X_{con}}}
\def\Xric{{X_{ric}}}
\def\xinit{{x_{I}}}
\def\xgoal{{x_{G}}}
\def\Xgoal{{X_{G}}}
\def\xcur{{x_{cur}}}
\def\xnew{{x_{new}}}

\def\B{{\cal B}}
\def\D{{\cal D}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\U{{\cal U}}
\def\W{{\cal W}}
\def\X{{\cal X}}

\def\Ufree{{\U_{free}}}

% Mapping for a singular simplex
\def\sing{{\sigma}}

\def\x{{ x}}
\def\u{{ u}}

\def\Uf{{\vec U}}
\def\Vf{{\vec V}}
\def\Wf{{\vec W}}
\def\Zf{{\vec Z}}

% Complexes
\def\Comp{{\cal K}}
\def\Cell{C}
\def\Simp{\Delta}

% van der Corput sequence
\def\vdc{{\nu}}
% General sequence
\def\genseq{{\alpha}}

\def\Re{{\mathbb{R}}}
\def\Com{{\mathbb{C}}}
\def\Z{{\mathbb{Z}}}
\def\S{{\mathbb{S}}}
\def\H{{\mathbb{H}}}
\def\Q{{\mathbb{Q}}}
\def\Nat{{\mathbb{N}}}
\def\RP{{\mathbb{RP}}}
\def\F{{\mathbb{F}}}
\def\T{{\mathbb{T}}}
\def\One{{\bf 1_G}}
\def\Ra{{\mathbb{A}}}
\def\Vs{{V}}

\def\Fcal{{\cal F}}

\def\q{{q}}

%% Randomized strategy
\def\urand{{w}}

\def\qq1{{q_1}}
\def\qk{{q_k}}
\def\qi{{q_i}}
\def\qkp1{{q_{k+1}}}
\def\qKp1{{q_{F}}}
\def\qKi{{q_{K+1}}}
\def\qKp1{{q_{F}}}
\def\qi{{q_{F}}}
\def\qxq1{{q_1}}

\def\uu1{{u_1}}
\def\uk{{u_k}}
\def\uK{{u_K}}
\def\ui{{u_i}}
\def\xk{{x_k}}
\def\xi{{x_i}}
\def\xkp1{{x_{k+1}}}
\def\xKp1{{x_{F}}}
\def\xKi{{x_{F}}}
\def\xq1{{x_1}}
\def\ukp1{{u_{k+1}}}
\def\thetak{{\theta_k}}

% These are backward actions
\def\bwactset{{U^{-1}}}
\def\bwact{u^{-1}}
\def\bwf{{f^{-1}}}

\def\octg{G^*}        % Optimal cost to go
\def\octc{C^*}        % Optimal cost to come 
\def\eoctg{G^*}       % expected Optimal cost to go
\def\eoctc{C^*}       % expected Optimal cost to come 
\def\woctg{G^*}       % worst-case Optimal cost to go
\def\wctg{G}       % worst-case cost to go
\def\woctc{C^*}       % worst-case Optimal cost to come 
\def\ctg{{G}}         % Cost-to-go   -- not necessarily optimal
\def\ctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\wctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\ctc{{C}}         % Cost-to-come -- not necessarily optimal
\def\ectg{\hat{G}^*}  % Estimated cost-to-go (A-star)
\def\ctgs{{g}}         % Cost-to-go for use in sampling chapter -- conflict with G
\def\exctg{G}       % expected Optimal cost to go
\def\exctgpl{G_\plan}       % expected Optimal cost to go
\def\exctc{C}       % expected Optimal cost to come 
\def\eoj{J^*}
\def\eojpl{J_\plan}
\def\qval{Q^*}
\def\aqval{\hat{Q}^*}
\def\qvalpl{Q_\plan}
\def\eectg{\hat{G}_\plan}

\def\cmean{\bar{c}}

\def\topi{{/\sim}} % Topological identification
\def\xb{{x_b}}

\def\Polys{{\cal P}}
\def\Poly{{P}}

%% 2D phase space for trajectory planning
\def\tphase{{S}}

%% Game theory
\def\Pa{{{\rm P}_1}}
\def\Pb{{{\rm P}_2}}
\def\Pc{{{\rm P}_3}}
\def\Pli{{{\rm P}_i}}
\def\Pn{{{\rm P}_n}}
\def\upperv{\overline{L}^*}
\def\lowerv{\underline{L}^*}
\def\ecost{{\bar{L}}}
\def\uppervm{\overline{\cal L}^*}
\def\lowervm{\underline{\cal L}^*}
\def\gamev{L^*}
\def\gameva{{L^*_a}}
\def\gamevb{{L^*_b}}
\def\gamevm{{\cal L}^*}

%% Plan definitions
\def\plan{\pi}
\def\fplan{\pi} %% Feedback
\def\iplan{\pi}
\def\pplan{\sigma} %% Partial plan
\def\planset{{\Pi}}
\def\fplanset{{\Pi}}

\def\argmax{\operatornamewithlimits{argmax}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\Pre{\operatorname{Pre}}
\def\Back{\operatorname{B}}
\def\SB{\operatorname{SB}}
\def\WB{\operatorname{WB}}
\def\Front{\operatorname{Front}}
\def\mymod{\operatorname{mod}}
\def\erf{\operatorname{erf}}
\def\hull{\operatorname{hull}}
\def\Front{\operatorname{Front}}
\def\atan2{\operatorname{atan2}}
\def\intfn{\operatorname{int}}
\def\dspan{\operatorname{span}}
\def\exp{\operatorname{exp}}
\def\adop{\operatorname{Ad}}
\def\clfn{\operatorname{cl}}
\def\Vor{\operatorname{Vor}}

\def\distr{{\triangle}}
\def\tdiff{{\Delta t}}
\def\lie{{\cal L}}
\def\phall{{\cal PH}}

\def\Cinfeq{{{\tilde C}^\infty}}

\def\truesp{\mbox{\sc{true }}}
\def\falsesp{\mbox{\sc{false }}}
\def\true{\mbox{\sc{true}}}
\def\false{\mbox{\sc{false}}}

\def\sccat{\mbox{\sc{cat}}}
\def\scdog{\mbox{\sc{dog}}}
\def\sctree{\mbox{\sc{tree}}}
\def\schouse{\mbox{\sc{house}}}

\def\qdot{{\dot q}}
\def\pdot{{\dot p}}
\def\qddot{{\ddot q}}
\def\qdddot{{q^{(3)}}}
\def\xdot{{\dot x}}
\def\xddot{{\ddot x}}
\def\yddot{{\ddot y}}
\def\ydot{{\dot y}}
\def\zdot{{\dot z}}
\def\xtdot{{{\dot x}_t}}
\def\ytdot{{{\dot y}_t}}
\def\thetadot{{\dot \theta}}
\def\thetaddot{{\ddot \theta}}
\def\adot{{\dot a}}
\def\bdot{{\dot b}}
\def\ceedot{{\dot c}}
\def\deedot{{\dot d}}
\def\fdot{{\dot f}}
\def\rdot{{\dot r}}
\def\sdot{{\dot s}}
\def\sddot{{\ddot s}}
\def\udot{{\dot u}}
\def\vdot{{\dot v}}
\def\wdot{{\dot w}}
\def\omegadot{{\dot \omega}}
\def\sigmadot{{\dot \omega}}
\def\phidot{{\dot \phi}}
\def\psidot{{\dot \psi}}
\def\alphadot{{\dot \alpha}}
\def\betadot{{\dot \beta}}
\def\gammadot{{\dot \gamma}}
\def\lambdadot{{\dot \lambda}}
\def\hdot{{\dot h}}
\def\gdot{{\dot g}}

\def\xtoq{{\kappa}}

\def\ustar{{u^*}}
\def\E{\operatorname{E}} %Expectation: $\E[X]$ (like \Pr)

\theoremstyle{plain}

%{\theorembodyfont{\rmfamily}\newtheorem{formulation}{Formulation}[chapter]}
%{\theorembodyfont{\rmfamily}\newtheorem{example}{Example}[chapter]}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Def}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{scenario}{Scenario}


\def\ds{\displaystyle\strut}
\def\idz{{\hspace{0.25in}}}

\def\disX{{\check X}}
\def\disx{{\check x}}
\def\disu{{\check u}}
\def\disU{{\check U}}
\def\disxgoal{{{\check x}_g}}
\def\disfplan{{\check \fplan}}
\def\disphi{{\check \phi}}

%% Dynamics
\def\force{{F}}
\def\moment{{N}}
\def\com{{p}} % Center of mass
\def\velcom{{\dot p}} % Center of mass
\def\acccom{{\ddot p}} % Center of mass
\def\mass{{m}}
\def\linmom{{D}} % Linear momentum
\def\angmom{{E}} % Angular momentum
\def\dens{{\sigma}}
\def\covfn{{\histx}} % Function for calculus of variations

\newcommand{\R}{{\mathcal R}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\qed}{\hfill $\blacksquare$ \hfill \\}


